Enhancing $t\bar{t}hh$ production through CP-violating top-Higgs interaction at the LHC, ILC and a 100 TeV collider

The measurement of Higgs self-coupling is one of the most crucial physics goals at the future colliders. At the LHC, the di-Higgs production is a main way to measure the Higgs trilinear coupling. As a complementary to the di-Higgs production, $t \bar{t} hh$ process may open a new avenue to measure di-Higgs physics at the LHC and a future 100 TeV $pp$ collider or a high energy $e^+e^-$ collider since the extra $t\bar t$ in the final states may efficiently suppress the backgrounds. However, such a kind of process is also controlled by the top-Higgs coupling. In this work, we investigate the impact of CP-violating top-Higgs coupling on $t\bar{t}hh$ production at the LHC, ILC and a 100 TeV hadron collider under the current Higgs data. Within 2$\sigma$ Higgs data allowed parameter region, we find that the cross section of $t\bar{t}hh$ at the LHC-14 TeV, ILC-1 TeV and VHE-LHC/SPPC-100 TeV can be enhanced up to 2.1 times the SM predictions. The future precise measurement of Higgs coupling will reveal the nature of top-Higgs interaction and improve the sensitivity of the determination of Higgs self-coupling through $t\bar{t}hh$ production.

==> bib.tex <==
\bibliographystyle{unsrt}
\begin{thebibliography}{9}
\bibitem{2012atlas}
  G.~Aad {\it et al.}  [ATLAS Collaboration],
  %``Observation of a new particle in the search for the Standard Model Higgs boson with the ATLAS detector at the LHC,''
  Phys.\ Lett.\ B {\bf 716}, 1 (2012), arXiv:1207.7214 [hep-ex].
  %%CITATION = ARXIV:1207.7214;%%
  %1339 citations counted in INSPIRE as of 12 Jul 2013kp

\bibitem{2012cms}
  S.~Chatrchyan {\it et al.}  [CMS Collaboration],
  %``Observation of a new boson at a mass of 125 GeV with the CMS experiment at the LHC,''
  Phys.\ Lett.\ B {\bf 716}, 30 (2012), arXiv:1207.7235 [hep-ex].
  %%CITATION = ARXIV:1207.7235;%%
  %1322 citations counted in INSPIRE as of 12 Jul 2013

\bibitem{2013atlas}The ATLAS Collaboration, ATLAS-CONF-2013-012; ATLAS-CONF-2013-034.

\bibitem{2013cms}The CMS Collaboration, CMS-PAS-HIG-13-001; CMS-PAS-HIG-13-005.

\bibitem{hh-sm} see examples in SM after 125 GeV Higgs boson,
  D.~Y.~Shao, C.~S.~Li, H.~T.~Li and J.~Wang,
  %``Threshold resummation effects in Higgs boson pair production at the LHC,''
  JHEP {\bf 1307}, 169 (2013)
  [arXiv:1301.1245 [hep-ph]];
  %%CITATION = ARXIV:1301.1245;%%
  %35 citations counted in INSPIRE as of 18 Aug 2014
  D.~de Florian and J.~Mazzitelli,
  %``Higgs Boson Pair Production at Next-to-Next-to-Leading Order in QCD,''
  Phys.\ Rev.\ Lett.\  {\bf 111}, 201801 (2013)
  [arXiv:1309.6594 [hep-ph]];
  %%CITATION = ARXIV:1309.6594;%%
  %30 citations counted in INSPIRE as of 18 Aug 2014
  X.~Li and M.~B.~Voloshin,
  %``Remarks on double Higgs boson production by gluon fusion at threshold,''
  Phys.\ Rev.\ D {\bf 89}, no. 1, 013012 (2014)
  [arXiv:1311.5156 [hep-ph]];
  %%CITATION = ARXIV:1311.5156;%%
  %4 citations counted in INSPIRE as of 18 Aug 2014
  J.~Grigo, K.~Melnikov and M.~Steinhauser,
  %``Virtual corrections to Higgs boson pair production in the large top quark mass limit,''
  arXiv:1408.2422 [hep-ph].
  %%CITATION = ARXIV:1408.2422;%%
  
\bibitem{Frederix:2014hta} 
  R.~Frederix, S.~Frixione, V.~Hirschi, F.~Maltoni, O.~Mattelaer, P.~Torrielli, E.~Vryonidou and M.~Zaro,
  %``Higgs pair production at the LHC with NLO and parton-shower effects,''
  Phys.\ Lett.\ B {\bf 732}, 142 (2014)
  [arXiv:1401.7340 [hep-ph]].
  %%CITATION = ARXIV:1401.7340;%%
  %12 citations counted in INSPIRE as of 18 Aug 2014
    
\bibitem{wengan}  
  L.~S.~Ling, R.~Y.~Zhang, W.~G.~Ma, L.~Guo, W.~H.~Li and X.~Z.~Li,
  %``NNLO QCD corrections to Higgs pair production via vector boson fusion at hadron colliders,''
  Phys.\ Rev.\ D {\bf 89}, no. 7, 073001 (2014)
  [arXiv:1401.7754 [hep-ph]].
  %%CITATION = ARXIV:1401.7754;%%
  %10 citations counted in INSPIRE as of 29 mar 2015

\bibitem{hh-mc1}
  U.~Baur, T.~Plehn and D.~L.~Rainwater,
  %``Determining the Higgs boson selfcoupling at hadron colliders,''
  Phys.\ Rev.\ D {\bf 67}, 033003 (2003)
  [hep-ph/0211224];
  %%CITATION = HEP-PH/0211224;%%
  %``Probing the Higgs selfcoupling at hadron colliders using rare decays,''
  Phys.\ Rev.\ D {\bf 69}, 053004 (2004)
  [hep-ph/0310056];
  %%CITATION = HEP-PH/0310056;%%
 J.~Baglio  {\it et al.},
  %``The measurement of the Higgs self-coupling at the LHC: theoretical status,''
  JHEP {\bf 1304}, 151 (2013)
  [arXiv:1212.5581 [hep-ph]].
  %%CITATION = ARXIV:1212.5581;%%

\bibitem{hh-mc2}
  D.~E.~Ferreira de Lima, A.~Papaefstathiou and M.~Spannowsky,
  %``Standard model Higgs boson pair production in the ( $ b\overline{b} $ )( $ b\overline{b} $ ) final state,''
  JHEP {\bf 1408}, 030 (2014)
  [arXiv:1404.7139 [hep-ph]];
  %%CITATION = ARXIV:1404.7139;%%
  D.~Wardrope, E.~Jansen, N.~Konstantinidis, B.~Cooper, R.~Falla and N.~Norjoharuddeen,
  %``Non-resonant Higgs pair production in the $b\overline{b}b\overline{b}$ final state at the LHC,''
  arXiv:1410.2794 [hep-ph].
  %%CITATION = ARXIV:1410.2794;%%
  
\bibitem{hh-mc3}
  M.~J.~Dolan, C.~Englert and M.~Spannowsky,
  %``Higgs self-coupling measurements at the LHC,''
  JHEP {\bf 1210}, 112 (2012)
  [arXiv:1206.5001 [hep-ph]];
  %%CITATION = ARXIV:1206.5001;%%
  F.~Goertz, A.~Papaefstathiou, L.~L.~Yang and J.~Zurita,
  %``Higgs Boson self-coupling measurements using ratios of cross sections,''
  JHEP {\bf 1306}, 016 (2013)
  [arXiv:1301.3492 [hep-ph]];
  %%CITATION = ARXIV:1301.3492;%%
  %64 citations counted in INSPIRE as of 15 Oct 2014  
  arXiv:1410.3471 [hep-ph];
  %%CITATION = ARXIV:1410.3471;%%
  %4 citations counted in INSPIRE as of 29 mar 2015    
  A.~Papaefstathiou, L.~L.~Yang and J.~Zurita,
  %``Higgs boson pair production at the LHC in the $b \bar{b} W^+ W^-$ channel,''
  Phys.\ Rev.\ D {\bf 87}, 011301 (2013)
  [arXiv:1209.1489 [hep-ph]];
  %%CITATION = ARXIV:1209.1489;%%
  F.~Goertz, A.~Papaefstathiou, L.~L.~Yang and J.~Zurita,
  %``Higgs Boson self-coupling measurements using ratios of cross sections,''
  JHEP {\bf 1306}, 016 (2013)
  [arXiv:1301.3492 [hep-ph]];
  %%CITATION = ARXIV:1301.3492;%%
  A.~J.~Barr, M.~J.~Dolan, C.~Englert and M.~Spannowsky,
  %``Di-Higgs final states augMT2ed -- selecting $hh$ events at the high luminosity LHC,''
  Phys.\ Lett.\ B {\bf 728}, 308 (2014)
  [arXiv:1309.6318 [hep-ph]];
  %%CITATION = ARXIV:1309.6318;%%
  %31 citations counted in INSPIRE as of 29 mar 2015    
  M.~J.~Dolan, C.~Englert, N.~Greiner and M.~Spannowsky,
  %``Further on up the road: $hhjj$ production at the LHC,''
  Phys.\ Rev.\ Lett.\  {\bf 112}, 101802 (2014)
  [arXiv:1310.1084 [hep-ph]];
  %%CITATION = ARXIV:1310.1084;%%
  P.~Maierh\"ofer and A.~Papaefstathiou,
  %``Higgs Boson pair production merged to one jet,''
  JHEP {\bf 1403}, 126 (2014)
  [arXiv:1401.0007 [hep-ph]];
  %%CITATION = ARXIV:1401.0007;%%
  V.~Barger, L.~L.~Everett, C.~B.~Jackson, A.~D.~Peterson and G.~Shaughnessy,
  %``New physics in resonant production of Higgs boson pairs,''
  Phys.\ Rev.\ Lett.\  {\bf 114}, no. 1, 011801 (2015)
  [arXiv:1408.0003 [hep-ph]];
  %%CITATION = ARXIV:1408.0003;%%
  %9 citations counted in INSPIRE as of 29 mar 2015  
  V.~Martin-Lozano, J.~M.~Moreno and C.~B.~Park,
  %``Resonant Higgs boson pair production in the $hh\rightarrow b\bar{b} \; WW \rightarrow b\bar{b} \ell^+ \nu \ell^- \bar\nu$ decay channel,''
  arXiv:1501.03799 [hep-ph];
  %%CITATION = ARXIV:1501.03799;%%
  %4 citations counted in INSPIRE as of 29 mar 2015
  Q.~Li, Z.~Li, Q.~S.~Yan and X.~Zhao,
  %``Probe Higgs boson pair production via the $3 \ell 2 j$ + missing $E_T$ mode,''
  arXiv:1503.07611 [hep-ph].
  %%CITATION = ARXIV:1503.07611;%% 
  

\bibitem{liuning}
  N.~Liu, S.~Hu, B.~Yang and J.~Han,
  %``Impact of top-Higgs couplings on Di-Higgs production at future colliders,''
  JHEP {\bf 1501}, 008 (2015)
  [arXiv:1408.4191 [hep-ph]].
  %%CITATION = ARXIV:1408.4191;%%
  %1 citations counted in INSPIRE as of 29 mar 2015

\bibitem{lilin}
  F.~Goertz, A.~Papaefstathiou, L.~L.~Yang and J.~Zurita,
  arXiv:1410.3471 [hep-ph].
  %%CITATION = ARXIV:1410.3471;%%
  %4 citations counted in INSPIRE as of 29 mar 2015    

\bibitem{liantao}
  A.~Pierce, J.~Thaler and L.~T.~Wang,
  %``Disentangling Dimension Six Operators through Di-Higgs Boson Production,''
  JHEP {\bf 0705}, 070 (2007)
  [hep-ph/0609049].
  %%CITATION = HEP-PH/0609049;%%
  %31 citations counted in INSPIRE as of 29 mar 2015

\bibitem{contino}
  R.~Contino, M.~Ghezzi, M.~Moretti, G.~Panico, F.~Piccinini and A.~Wulzer,
  %``Anomalous Couplings in Double Higgs Production,''
  JHEP {\bf 1208}, 154 (2012)
  [arXiv:1205.5444 [hep-ph]].
  %%CITATION = ARXIV:1205.5444;%%
  %33 citations counted in INSPIRE as of 18 Aug 2014

\bibitem{nishiwaki}
  K.~Nishiwaki, S.~Niyogi and A.~Shivaji,
  %``$ttH$ Anomalous Coupling in Double Higgs Production,''
  JHEP {\bf 1404}, 011 (2014)
  [arXiv:1309.6907 [hep-ph]];
  %%CITATION = ARXIV:1309.6907;%%
  %6 citations counted in INSPIRE as of 18 Aug 20

\bibitem{ian}  
  C.~R.~Chen and I.~Low,
  %``A Double Take on New Physics in Double Higgs Production,''
  arXiv:1405.7040 [hep-ph];
  %%CITATION = ARXIV:1405.7040;%%
  %4 citations counted in INSPIRE as of 18 Aug 2014

\bibitem{das}
  G.~Bhattacharyya, D.~Das and P.~B.~Pal,
  %``Modified Higgs couplings and unitarity violation,''
  Phys.\ Rev.\ D {\bf 87}, 011702 (2013)
  [arXiv:1212.4651 [hep-ph]].
  %%CITATION = ARXIV:1212.4651;%%
  %9 citations counted in INSPIRE as of 22 Aug 2014
  
\bibitem{tth-atlas}
ATLAS Collaboration [ATLAS Collaboration], ATLAS-CONF-2014-011.

\bibitem{tth-cms}
CMS Collaboration [CMS Collaboration], CMS-PAS-HIG-14-010.

\bibitem{tth-old}
  W.~J.~Marciano and F.~E.~Paige,
  %``Associated production of Higgs bosons with t anti-t pairs,''
  Phys.\ Rev.\ Lett.\  {\bf 66}, 2433 (1991);
  %%CITATION = PRLTA,66,2433;%%
  %137 citations counted in INSPIRE as of 24 May 2014
  J.~Dai, J.~F.~Gunion and R.~Vega,
  %``Using b tagging to detect t anti-t Higgs production with Higgs ---> b anti-b,''
  Phys.\ Rev.\ Lett.\  {\bf 71}, 2699 (1993)  [hep-ph/9306271];
  %%CITATION = HEP-PH/9306271;%%
  %62 citations counted in INSPIRE as of 24 May 2014
  J.~Goldstein, C.~S.~Hill, J.~Incandela, S.~J.~Parke, D.~L.~Rainwater and D.~Stuart,
  %``$p\bar{p}\to t\bar{t}H$: A Discovery mode for the Higgs boson at the Tevatron,''
  Phys.\ Rev.\ Lett.\  {\bf 86}, 1694 (2001)  [hep-ph/0006311];
  %%CITATION = HEP-PH/0006311;%%
  %55 citations counted in INSPIRE as of 24 May 2014
  A.~Belyaev and L.~Reina,
  %``pp ---> t anti-t H, H ---> tau+ tau-: Toward a model independent determination of the Higgs boson couplings at the LHC,''
  JHEP {\bf 0208}, 041 (2002)  [hep-ph/0205270];
  %%CITATION = HEP-PH/0205270;%%
  %101 citations counted in INSPIRE as of 24 May 2014
  F.~Maltoni, D.~L.~Rainwater and S.~Willenbrock,
  %``Measuring the top quark Yukawa coupling at hadron colliders via $t\bar{t}H,H\to W^+W^-$,''
  Phys.\ Rev.\ D {\bf 66}, 034022 (2002)  [hep-ph/0202205];
  %%CITATION = HEP-PH/0202205;%%
  %62 citations counted in INSPIRE as of 24 May 2014
  V.~Drollinger, T.~Muller and D.~Denegri,
  %``Searching for Higgs bosons in association with top quark pairs in the H0 ---> b anti-b decay mode,''
  hep-ph/0111312;
  %%CITATION = HEP-PH/0111312;%%
  %87 citations counted in INSPIRE as of 24 May 2014
  W.~Beenakker, S.~Dittmaier, M.~Kramer, B.~Plumper, M.~Spira and P.~M.~Zerwas,
  %``NLO QCD corrections to t anti-t H production in hadron collisions,''
   Nucl.\ Phys.\ B {\bf 653}, 151 (2003)  [hep-ph/0211352].
   %%CITATION = HEP-PH/0211352;%%
   %250 citations counted in INSPIRE as of 24 May 2014


\bibitem{tth-new}
  P.~Agrawal, S.~Bandyopadhyay and S.~P.~Das,
  %``Multilepton Signatures of the Higgs Boson through its Production in Association with a Top-quark Pair,''
  Phys.\ Rev.\ D {\bf 88}, 093008 (2013)  [arXiv:1308.3043 [hep-ph]];
  %%CITATION = ARXIV:1308.3043;%%
  %5 citations counted in INSPIRE as of 24 May 2014
  S.~Biswas, R.~Frederix, E.~Gabrielli and B.~Mele,
  %``Enhancing the ttH signal through top-quark spin polarization effects at the LHC,''
  arXiv:1403.1790 [hep-ph];
  %%CITATION = ARXIV:1403.1790;%%
  M.~V.~Garzelli, A.~Kardos, C.~G.~Papadopoulos and Z.~Trocsanyi,
  %``Standard Model Higgs boson production in association with a top anti-top pair at NLO with parton showering,''
  Europhys.\ Lett.\  {\bf 96}, 11001 (2011)  [arXiv:1108.0387 [hep-ph]];
  %%CITATION = ARXIV:1108.0387;%%
  %34 citations counted in INSPIRE as of 24 May 2014
  R.~Frederix, S.~Frixione, V.~Hirschi, F.~Maltoni, R.~Pittau and P.~Torrielli,
  %``Scalar and pseudoscalar Higgs production in association with a top-antitop pair,''
  Phys.\ Lett.\ B {\bf 701}, 427 (2011)  [arXiv:1104.5613 [hep-ph]];
  %%CITATION = ARXIV:1104.5613;%%
  %58 citations counted in INSPIRE as of 24 May 2014
  C.~Degrande, J.~M.~Gerard, C.~Grojean, F.~Maltoni and G.~Servant,
  %``Probing Top-Higgs Non-Standard Interactions at the LHC,''
  JHEP {\bf 1207}, 036 (2012)  [Erratum-ibid.\  {\bf 1303}, 032 (2013)]  [arXiv:1205.1065 [hep-ph]];
  %%CITATION = ARXIV:1205.1065;%%
  %25 citations counted in INSPIRE as of 24 May 2014
  D.~Curtin, J.~Galloway and J.~G.~Wacker,
  %``Measuring the tth coupling from SSDL+2b measurements,''
  Phys.\ Rev.\ D {\bf 88}, 093006 (2013)  [arXiv:1306.5695 [hep-ph]];
  %%CITATION = ARXIV:1306.5695;%%
  %11 citations counted in INSPIRE as of 24 May 2014
  J.~Adelman, A.~Loginov, P.~Tipton and J.~Vasquez,
  %``Study of $t\bar{t}H$ ($H \to \mu^+ \bar{\mu}^-$) in the three lepton channel at $\sqrt{s}=14$ TeV; A Snowmass white paper,''
  arXiv:1310.1132 [hep-ex];
  %%CITATION = ARXIV:1310.1132;%%
  %3 citations counted in INSPIRE as of 24 May 2014
  F.~Boudjema, R.~M.~Godbole, D.~Guadagnoli and K.~A.~Mohan,
  %``Lab-frame observables for probing the top-Higgs interaction,''
  arXiv:1501.03157 [hep-ph];
  %%CITATION = ARXIV:1501.03157;%%
  %4 citations counted in INSPIRE as of 29 mar 2015
  X.~G.~He, G.~N.~Li and Y.~J.~Zheng,
  %``Probing Higgs Boson $CP$ Properties with $t\bar{t}H$ at the LHC and the 100 TeV $pp$ Collider,''
  arXiv:1501.00012 [hep-ph].
  %%CITATION = ARXIV:1501.00012;%%
  %3 citations counted in INSPIRE as of 29 mar 2015  

\bibitem{Heinemeyer:2013tqa}
  S.~Heinemeyer {\it et al.}  [LHC Higgs Cross Section Working Group Collaboration],
  %``Handbook of LHC Higgs Cross Sections: 3. Higgs Properties,''
  arXiv:1307.1347 [hep-ph].
  %%CITATION = ARXIV:1307.1347;%%
  %321 citations counted in INSPIRE as of 29 mar 2015

\bibitem{atlas:tth_gaga}
The ATLAS collaboration, ATLAS-CONF-2014-043.

\bibitem{Khachatryan:2014qaa} 
  V.~Khachatryan {\it et al.}  [CMS Collaboration],
  %``Search for the associated production of the Higgs boson with a top-quark pair,''
  JHEP {\bf 1409}, 087 (2014)
  [Erratum-ibid.\  {\bf 1410}, 106 (2014)]
  [arXiv:1408.1682 [hep-ex]].
  %%CITATION = ARXIV:1408.1682;%%
  %24 citations counted in INSPIRE as of 29 mar 2015


\bibitem{thj-old}
  G.~Bordes and B.~van Eijk,
  %``On the associate production of a neutral intermediate mass Higgs boson with a single top quark at the LHC and SSC,''
  Phys.\ Lett.\ B {\bf 299}, 315 (1993);
  %%CITATION = PHLTA,B299,315;%%
  %15 citations counted in INSPIRE as of 24 May 2014
  A.~Ballestrero and E.~Maina,
  %``t anti-b H production for an intermediate mass Higgs,''
  Phys.\ Lett.\ B {\bf 299}, 312 (1993);
  %%CITATION = PHLTA,B299,312;%%
  %16 citations counted in INSPIRE as of 24 May 2014
  W.~J.~Stirling and D.~J.~Summers,
  %``Production of an intermediate mass Higgs boson in association with a single top quark at LHC and SSC,''
  Phys.\ Lett.\ B {\bf 283}, 411 (1992);
  %%CITATION = PHLTA,B283,411;%%
  %19 citations counted in INSPIRE as of 24 May 2014
  J.~L.~Diaz-Cruz and O.~A.~Sampayo,
  %``Associated production of the Higgs boson with t anti-b at hadron colliders,''
  Phys.\ Lett.\ B {\bf 276}, 211 (1992);
  %%CITATION = PHLTA,B276,211;%%
  %10 citations counted in INSPIRE as of 24 May 2014
  T.~M.~P.~Tait and C.-P.~Yuan,
  %``Single top quark production as a window to physics beyond the standard model,''
  Phys.\ Rev.\ D {\bf 63}, 014018 (2000)
  [hep-ph/0007298];
  %%CITATION = HEP-PH/0007298;%%
  %291 citations counted in INSPIRE as of 18 Aug 2014
  F.~Maltoni, K.~Paul, T.~Stelzer and S.~Willenbrock,
  %``Associated production of Higgs and single top at hadron colliders,''
  Phys.\ Rev.\ D {\bf 64}, 094023 (2001)  [hep-ph/0106293];
  %%CITATION = HEP-PH/0106293;%%
  %35 citations counted in INSPIRE as of 24 May 2014
  G.~R.~Lu and L.~Wu,
  %``Flavor-changing neutral-current production of t anti-c in association with a neutral top-Higgs at LHC in the topcolor-assisted technicolor model,''
  Chin.\ Phys.\ Lett.\  {\bf 27}, 031401 (2010).
  %%CITATION = CPLEE,27,031401;%%
  %6 citations counted in INSPIRE as of 29 mar 2015
  
\bibitem{thj-new}
  P.~Agrawal, S.~Mitra and A.~Shivaji,
  %``Effect of Anomalous Couplings on the Associated Production of a Single Top Quark and a Higgs Boson at the LHC,''
  JHEP {\bf 1312}, 077 (2013)
  [arXiv:1211.4362 [hep-ph]];
  %%CITATION = ARXIV:1211.4362;%%
  %9 citations counted in INSPIRE as of 16 Oct 2014
  Y.~Wang, F.~P.~Huang, C.~S.~Li, B.~H.~Li, D.~Y.~Shao and J.~Wang,
  %``Constraints on flavor-changing neutral-current $Htq$ couplings from the signal of $tH$ associated production with QCD next-to-leading order accuracy at the LHC,''
  Phys.\ Rev.\ D {\bf 86}, 094014 (2012)
  [arXiv:1208.2902 [hep-ph]].
  %%CITATION = ARXIV:1208.2902;%%
  %5 citations counted in INSPIRE as of 18 Aug 2014
  M.~Farina, C.~Grojean, F.~Maltoni, E.~Salvioni and A.~Thamm,
  %``Lifting degeneracies in Higgs couplings using single top production in association with a Higgs boson,''
  JHEP {\bf 1305}, 022 (2013)  [arXiv:1211.3736 [hep-ph]].
  %%CITATION = ARXIV:1211.3736;%%
  %32 citations counted in INSPIRE as of 24 May 2014
  S.~Biswas, E.~Gabrielli and B.~Mele,
  %``Single top and Higgs associated production as a probe of the Htt coupling sign at the LHC,''
  JHEP {\bf 1301}, 088 (2013)  [arXiv:1211.0499 [hep-ph]].
  %%CITATION = ARXIV:1211.0499;%%
  %26 citations counted in INSPIRE as of 24 May 2014
  J.~Ellis, D.~S.~Hwang, K.~Sakurai and M.~Takeuchi,
  %``Disentangling Higgs-Top Couplings in Associated Production,''
  JHEP {\bf 1404}, 004 (2014)  [arXiv:1312.5736 [hep-ph]].  %%CITATION = ARXIV:1312.5736;%%  %9 citations counted in INSPIRE as of 24 May 2014
  C.~Englert and E.~Re,
  %``Bounding the top Yukawa with Higgs-associated single-top production,''
  Phys.\ Rev.\ D {\bf 89}, 073020 (2014)  [arXiv:1402.0445 [hep-ph]];
  %%CITATION = ARXIV:1402.0445;%%
  %3 citations counted in INSPIRE as of 26 May 2014
  J.~Chang, K.~Cheung, J.~S.~Lee and C.~-T.~Lu,
  %``Probing the Top-Yukawa Coupling in Associated Higgs production with a Single Top Quark,''
  JHEP {\bf 1405}, 062 (2014)  [arXiv:1403.2053 [hep-ph]];
  %%CITATION = ARXIV:1403.2053;%%
  %1 citations counted in INSPIRE as of 24 May 2014
  A.~Kobakhidze, L.~Wu and J.~Yue,
  %``Anomalous Top-Higgs Couplings and Top Polarisation in Single Top and Higgs Associated Production at the LHC,''
  JHEP {\bf 1410}, 100 (2014)
  [arXiv:1406.1961 [hep-ph]];
  %%CITATION = ARXIV:1406.1961;%%
  %10 citations counted in INSPIRE as of 29 mar 2015
  L.~Wu,
  %``Enhancing $thj$ Production from Top-Higgs FCNC Couplings,''
  JHEP {\bf 1502}, 061 (2015)
  [arXiv:1407.6113 [hep-ph]];
  %%CITATION = ARXIV:1407.6113;%%
  %5 citations counted in INSPIRE as of 29 mar 2015
  J.~Yue,
  %``$\mathcal{CP}$-violating top-Higgs coupling and top polarisation in the diphoton decay of the $thj$ channel at the LHC,''
  arXiv:1410.2701 [hep-ph];
  %%CITATION = ARXIV:1410.2701;%%
  %1 citations counted in INSPIRE as of 29 mar 2015
  B.~Yang, J.~Han and N.~Liu,
  %``Associated production of single top and Higgs at the LHC in the littlest Higgs model with T-parity,''
  arXiv:1412.2927 [hep-ph].
  %%CITATION = ARXIV:1412.2927;%%

\bibitem{thj-cms}
CMS Collaboration [CMS Collaboration], CMS-PAS-HIG-14-001.


\bibitem{tthh1}
  C.~Englert, F.~Krauss, M.~Spannowsky and J.~Thompson,
  %``Di-Higgs phenomenology in $t\bar{t}hh$: The forgotten channel,''
  Phys.\ Lett.\ B {\bf 743}, 93 (2015)
  [arXiv:1409.8074 [hep-ph]].
  %%CITATION = ARXIV:1409.8074;%%
  %3 citations counted in INSPIRE as of 29 mar 201

\bibitem{tthh2}
  T.~Liu and H.~Zhang,
  %``Measuring Di-Higgs Physics via the $t \bar t hh \to t \bar t b \bar bb\bar b$ Channel,''
  arXiv:1410.1855 [hep-ph].
  %%CITATION = ARXIV:1410.1855;%%
  %1 citations counted in INSPIRE as of 29 mar 2015


\bibitem{ilc-white}
  D.~M.~Asner, T.~Barklow, C.~Calancha, K.~Fujii, N.~Graf, H.~E.~Haber, A.~Ishikawa and S.~Kanemura {\it et al.},
  %``ILC Higgs White Paper,''
  arXiv:1310.0763 [hep-ph].
  %%CITATION = ARXIV:1310.0763;%%
  %49 citations counted in INSPIRE as of 18 Aug 2014

\bibitem{hf} see recent examples at $e^+e^-$ colliders:
  N.~Craig, M.~Farina, M.~McCullough and M.~Perelstein,
  %``Precision Higgsstrahlung as a Probe of New Physics,''
  arXiv:1411.0676 [hep-ph];
  %%CITATION = ARXIV:1411.0676;%%
  %5 citations counted in INSPIRE as of 29 mar 2015
  J.~Cao, C.~Han, J.~Ren, L.~Wu, J.~M.~Yang and Y.~Zhang,
  %``SUSY effects in Higgs productions at high energy $e^+e^-$ colliders,''
  arXiv:1410.1018 [hep-ph];
  %%CITATION = ARXIV:1410.1018;%%
  %3 citations counted in INSPIRE as of 29 mar 2015  
  V.~Barger, L.~L.~Everett, H.~E.~Logan and G.~Shaughnessy,
  %``Scrutinizing h(125) in Two Higgs Doublet Models at the LHC, ILC, and Muon Collider,''  P
  hys.\ Rev.\ D {\bf 88}, 115003 (2013)  [arXiv:1308.0052 [hep-ph]];
  %%CITATION = ARXIV:1308.0052;%%  %22 citations counted in INSPIRE as of 24 May 2014
  N.~Liu, J.~Ren, L.~Wu, P.~Wu and J.~M.~Yang,
  %``Full one-loop electroweak corrections to $e^+e^- \to ZH\gamma$ at a Higgs factory,''
  JHEP {\bf 1404}, 189 (2014)  [arXiv:1311.6971 [hep-ph]];
  %%CITATION = ARXIV:1311.6971;%%
  %2 citations counted in INSPIRE as of 24 May 2014
  Z.~Heng, L.~Shang and P.~Wan,
  %``Pair production of a 125 GeV Higgs boson in MSSM and NMSSM at the ILC,''
  JHEP {\bf 1310}, 047 (2013)  [arXiv:1306.0279 [hep-ph]];
  %%CITATION = ARXIV:1306.0279;%%
  %5 citations counted in INSPIRE as of 24 May 2014
  S.~L.~Hu, N.~Liu, J.~Ren and L.~Wu,
  %``Revisiting Associated Production of 125 GeV Higgs Boson with a Photon at a Higgs Factory,''
  J.\ Phys.\ G {\bf 41}, no. 12, 125004 (2014)
  [arXiv:1402.3050 [hep-ph]];
  %%CITATION = ARXIV:1402.3050;%%
  %6 citations counted in INSPIRE as of 29 mar 2015
  L.~Wang and X.~-F.~Han,
  %``Study of the heavy CP-even Higgs with mass 125 GeV in two-Higgs-doublet models at the LHC and ILC,''
  arXiv:1404.7437 [hep-ph];
  %%CITATION = ARXIV:1404.7437;%%
  %1 citations counted in INSPIRE as of 24 May 2014
  C.~Han, A.~Kobakhidze, N.~Liu, L.~Wu and B.~Yang,
  %``Constraining Top partner and Naturalness at the LHC and TLEP,''
  arXiv:1405.1498 [hep-ph];
  %%CITATION = ARXIV:1405.1498;%%
  J.~Cao, Z.~Heng, D.~Li, L.~Shang and P.~Wu,
  %``Higgs-strahlung production process e^+ e^- \to Z h at the future Higgs factory in the Minimal Dilaton Model,''
  arXiv:1405.4489 [hep-ph];
  %%CITATION = ARXIV:1405.4489;%%
  B.~Yang, Z.~Liu, N.~Liu and J.~Han,
  %``Double Higgs production in the littlest Higgs Model with T-parity at high energy $e^{+}e^{-}$ Colliders,''
  Eur.\ Phys.\ J.\ C {\bf 74}, no. 12, 3203 (2014)
  [arXiv:1408.4295 [hep-ph]].
  %%CITATION = ARXIV:1408.4295;%%

\bibitem{ilc-rr}
  I.~F.~Ginzburg, G.~L.~Kotkin, V.~G.~Serbo and V.~I.~Telnov,
  %``Production of High-Energy Colliding gamma gamma and gamma e Beams with a High Luminosity at Vlepp Accelerators,''
  JETP Lett.\  {\bf 34}, 491 (1981)
  [Pisma Zh.\ Eksp.\ Teor.\ Fiz.\  {\bf 34}, 514 (1981)].
  %%CITATION = JTPLA,34,491;%%
  %219 citations counted in INSPIRE as of 18 Aug 2014

\bibitem{ee-tthh}
  A.~Gutierrez-Rodriguez, M.~A.~Hernandez-Ruiz, O.~A.~Sampayo, A.~Chubykalo and A.~Espinoza-Garrido,
  %``The Triple Higgs Boson Self-Coupling at Future Linear e+e- Colliders Energies: ILC and CLIC,''
  J.\ Phys.\ Soc.\ Jap.\  {\bf 77}, 094101 (2008)
  [arXiv:0807.0663 [hep-ph]].
  %%CITATION = ARXIV:0807.0663;%%
  %8 citations counted in INSPIRE as of 29 mar 2015

\bibitem{aa-tthh}
  A.~Gutierrez-Rodriguez, J.~Peressutti and O.~A.~Sampayo,
  %``Higgs Boson Self-Coupling at High Energy $\gamma \gamma$ Collider,''
  J.\ Phys.\ G {\bf 38}, 095002 (2011)
  [arXiv:1107.0245 [hep-ph]].
  %%CITATION = ARXIV:1107.0245;%%
  %1 citations counted in INSPIRE as of 29 mar 2015


\bibitem{zupan}
  J.~Brod, U.~Haisch and J.~Zupan,
  %``Constraints on CP-violating Higgs couplings to the third generation,''
  JHEP {\bf 1311}, 180 (2013)  [arXiv:1310.1385 [hep-ph]].
  %%CITATION = ARXIV:1310.1385;%%
  %11 citations counted in INSPIRE as of 25 May 2014

\bibitem{higgssignals}
  P.~Bechtle {\it et al.},
  %``$HiggsSignals$: Confronting arbitrary Higgs sectors with measurements at the Tevatron and the LHC,''
  Eur.\ Phys.\ J.\ C {\bf 74}, 2711 (2014)  [arXiv:1305.1933 [hep-ph]];
  %%CITATION = ARXIV:1305.1933;%%
  %33 citations counted in INSPIRE as of 23 Apr 2014
  P.~Bechtle {\it et al.},
  %``HiggsBounds: Confronting Arbitrary Higgs Sectors with Exclusion Bounds from LEP and the Tevatron,''
  Comput.\ Phys.\ Commun.\  {\bf 181}, 138 (2010)  [arXiv:0811.4169 [hep-ph]].
  %%CITATION = ARXIV:0811.4169;%%
  %161 citations counted in INSPIRE as of 23 Apr 2014
  

\bibitem{top_cp_review}
  D.~Atwood, S.~Bar-Shalom, G.~Eilam and A.~Soni,
  %``CP violation in top physics,''
  Phys.\ Rept.\  {\bf 347}, 1 (2001)  [hep-ph/0006032];
  %%CITATION = HEP-PH/0006032;%%
  %124 citations counted in INSPIRE as of 25 May 2014
  A.~Kobakhidze,
  %``Standard Model with a distorted Higgs sector and the enhanced Higgs diphoton decay rate,''
  arXiv:1208.5180 [hep-ph].
  %%CITATION = ARXIV:1208.5180;%%
  %13 citations counted in INSPIRE as of 25 May 2014


\bibitem{pdg}
J. Beringer {\it et al.}, Particle Data Group, Phys.\ Rev. \ D {\bf
86}, 010001 (2012) and 2013 partial update for the 2014 edition.

\bibitem{cteq}
  H.~L.~Lai, M.~Guzzi, J.~Huston, Z.~Li, P.~M.~Nadolsky, J.~Pumplin and C.-P.~Yuan,
  %``New parton distributions for collider physics,''
  Phys.\ Rev.\ D {\bf 82}, 074024 (2010)
  [arXiv:1007.2241 [hep-ph]].
  %%CITATION = ARXIV:1007.2241;%%
  %1220 citations counted in INSPIRE as of 29 mar 2015


\bibitem{calchep}
  A.~Belyaev, N.~D.~Christensen and A.~Pukhov,
  %``CalcHEP 3.4 for collider physics within and beyond the Standard Model,''
  Comput.\ Phys.\ Commun.\  {\bf 184}, 1729 (2013)
  [arXiv:1207.6082 [hep-ph]].
  %%CITATION = ARXIV:1207.6082;%%
  %206 citations counted in INSPIRE as of 29 mar 2015

\bibitem{photon collider}
I. F. Ginzburg {\it et al.}, Nucl. Instrum 219, 5 (1984);
V. I. Telnov,  Nucl. Instrum. Meth. 294, 72 (1990).



\end{thebibliography}


